XPath Node Selection over Grammar-Compressed Trees

XML document markup is highly repetitive and therefore well compressible using grammar-based compression. Downward, navigational XPath can be executed over grammar-compressed trees in PTIME: the query is translated into an automaton which is executed in one pass over the grammar. This result is well-known and has been mentioned before. Here we present precise bounds on the time complexity of this problem, in terms of big-O notation. For a given grammar and XPath query, we consider three different tasks: (1) to count the number of nodes selected by the query, (2) to materialize the pre-order numbers of the selected nodes, and (3) to serialize the subtrees at the selected nodes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{S. Maneth (Ed.): Workshop on Trends in Tree\\
Automata and Tree Transducers (TTATT 2013).\\
EPTCS 134, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.134.5}{10.4204/EPTCS.134.5}}

